A Computer Vision Problem in Flatland

When is it possible to project two sets of labeled points lying in a pair of projective planes to the same image on a projective line? We give a complete answer to this question and describe the loci of the projection centers that enable a common image. In particular, we find that there exists a solution to this problem if and only if these two sets are themselves images of a common pointset in projective space.

==> images/m0-is-sum-of-others.tex <==
\definecolor{yqyqyq}{rgb}{0.5019607843137255,0.5019607843137255,0.5019607843137255}
\definecolor{xdxdff}{rgb}{0.49019607843137253,0.49019607843137253,1.}
\definecolor{uuuuuu}{rgb}{0.26666666666666666,0.26666666666666666,0.26666666666666666}

\def\ONE#1#2{({0+#1},{1.7393550206807582+#2})}
\def\TWO#1#2{(1.0042170894063625+#1,1.7393550206807578+#2)}
\def\THREE#1#2{(1.5063256341095437+#1,0.8696775103403789+#2)}
\def\FOUR#1#2{({1.0042170894063625+#1},{0.+#2})}
\def\FIVE#1#2{(0.+#1,0.+#2)}
\def\SIX#1#2{(-0.5021085447031814+#1,0.8696775103403797+#2)}

\def\HEXAGON#1#2{
	\fill[line width=1.0pt,dotted,color=yqyqyq,fill=yqyqyq,fill opacity=0.10000000149011612] 
	(0.+#1, 0.+#2) -- (1.0042170894063625 +#1, 0.+#2) -- (1.5063256341095437+#1, 0.8696775103403789+#2) -- 
	(1.0042170894063625+#1, 1.7393550206807578+#2) -- (0.+#1, 1.7393550206807582+#2) -- (-0.5021085447031814+#1, 0.8696775103403797+#2) 
	-- cycle;
	
	\begin{scriptsize}	    
    \fill  (0.+#1,1.7393550206807582+#2) circle (1.5pt);
    	\draw (-0.1+#1, 2.0+#2) node {1};
    \fill (1.0042170894063625+#1,1.7393550206807578+#2) circle (1.5pt);
    	\draw (1.15+#1, 2.0+#2) node {2};
     \fill  (1.5063256341095437+#1,0.8696775103403789+#2) circle (1.5pt);
   	 \draw (1.7+#1, 0.86+#2) node {3};
    \fill  (1.0042170894063625+#1,0.+#2) circle (1.5pt);
    \draw  (1.15+#1, -0.15+#2) node {4};
    \fill  (0.+#1,0.+#2) circle (1.5pt);
  	  \draw (-0.1+#1, -0.15+#2) node {5};
   \fill (-0.5021085447031814+#1,0.8696775103403797+#2) circle (1.5pt);
	    \draw (-0.7+#1, 0.86+#2) node {6};
	 \end{scriptsize}
	}
\begin{tikzpicture}[scale=0.8,
	line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]

\HEXAGON{0}{0}
	\draw[->] \ONE{0}{0} -- \TWO{0}{0};
	\draw[->] \FOUR{0}{0} -- \FIVE{0}{0};
	\draw[->] \THREE{0}{0} -- \SIX{0}{0};
\HEXAGON{3}{0}
	\draw[->] \ONE{3}{0} -- \TWO{3}{0};
	\draw[->] \FIVE{3}{0} -- \SIX{3}{0};
	\draw[->] \THREE{3}{0} -- \FOUR{3}{0};
\HEXAGON{6}{0}
	\draw[->] \ONE{6}{0} -- \FOUR{6}{0};
	\draw[->] \TWO{6}{0} -- \THREE{6}{0};
	\draw[->] \FIVE{6}{0} -- \SIX{6}{0};
\HEXAGON{9}{0}
	\draw[->] \ONE{9}{0} -- \SIX{9}{0};
	\draw[->] \FOUR{9}{0} -- \FIVE{9}{0};
	\draw[->] \TWO{9}{0} -- \THREE{9}{0};
\HEXAGON{12}{0}
	\draw[->] \ONE{12}{0} -- \SIX{12}{0};
	\draw[->] \TWO{12}{0} -- \FIVE{12}{0};
	\draw[->] \THREE{12}{0} -- \FOUR{12}{0};


\HEXAGON{0}{3}
	\draw[->] \ONE{0}{3} -- \TWO{0}{3};
	\draw[->] \FOUR{0}{3} -- \FIVE{0}{3};
	\draw[->] \THREE{0}{3} -- \SIX{0}{3};
\HEXAGON{4.5}{3}
	\draw[->] \ONE{4.5}{3} -- \THREE{4.5}{3};
	\draw[->] \TWO{4.5}{3} -- \FOUR{4.5}{3};
	\draw[->] \FIVE{4.5}{3} -- \SIX{4.5}{3};
\HEXAGON{10.5}{3}
	\draw[->] \ONE{10.5}{3} -- \SIX{10.5}{3};
	\draw[->] \TWO{10.5}{3} -- \FOUR{10.5}{3};
	\draw[->] \THREE{10.5}{3} -- \FIVE{10.5}{3};


\HEXAGON{0}{6}
	\draw[->] \ONE{0}{6} -- \TWO{0}{6};
	\draw[->] \FOUR{0}{6} -- \FIVE{0}{6};
	\draw[->] \THREE{0}{6} -- \SIX{0}{6};
\HEXAGON{7.5}{6}
	\draw[->] \ONE{7.5}{6} -- \FIVE{7.5}{6};
	\draw[->] \TWO{7.5}{6} -- \FOUR{7.5}{6};
	\draw[->] \THREE{7.5}{6} -- \SIX{7.5}{6};

\HEXAGON{-4}{6}
	\draw[->] \ONE{-4}{6} -- \FOUR{-4}{6};
	\draw[->] \TWO{-4}{6} -- \FIVE{-4}{6};
	\draw[->] \THREE{-4}{6} -- \SIX{-4}{6};


\begin{scriptsize}
\draw (-1.5, 6.86) node {$=$};
\draw (-1.5, 3.86) node {$=$};
\draw (-1.5, 0.86) node {$=$};

\draw (4, 6.86) node {$+$};
\draw (2.5, 3.86) node {$+$};
\draw (8, 3.86) node {$+$};

\draw (2, 1.1) node {$+$};
\draw (5, 1.1) node {$+$};
\draw (8, 1.1) node {$+$};
\draw (11, 1.1) node {$+$};

\draw (-3.5, 5.25) node {$m_0$};
\draw (0.5, -0.75) node {$m_5$};
\draw (3.5, -0.75) node {$m_1$};
\draw (6.5, -0.75) node {$m_3$};
\draw (9.5, -0.75) node {$m_2$};
\draw (12.5, -0.75) node {$m_4$};

\end{scriptsize}
\end{tikzpicture}
